Conditionally optimal approximation algorithms for the girth of a directed graph

It is known that a better than $2$-approximation algorithm for the girth in dense directed unweighted graphs needs $n^{3-o(1)}$ time unless one uses fast matrix multiplication. Meanwhile, the best known approximation factor for a combinatorial algorithm running in $O(mn^{1-\epsilon})$ time (by Chechik et al.) is $3$. Is the true answer $2$ or $3$? The main result of this paper is a (conditionally) tight approximation algorithm for directed graphs. First, we show that under a popular hardness assumption, any algorithm, even one that exploits fast matrix multiplication, would need to take at least $mn^{1-o(1)}$ time for some sparsity $m$ if it achieves a $(2-\epsilon)$-approximation for any $\epsilon>0$. Second we give a $2$-approximation algorithm for the girth of unweighted graphs running in $\tilde{O}(mn^{3/4})$ time, and a $(2+\epsilon)$-approximation algorithm (for any $\epsilon>0$) that works in weighted graphs and runs in $\tilde{O}(m\sqrt n)$ time. Our algorithms are combinatorial. We also obtain a $(4+\epsilon)$-approximation of the girth running in $\tilde{O}(mn^{\sqrt{2}-1})$ time, improving upon the previous best $\tilde{O}(m\sqrt n)$ running time by Chechik et al. Finally, we consider the computation of roundtrip spanners. We obtain a $(5+\epsilon)$-approximate roundtrip spanner on $\tilde{O}(n^{1.5}/\epsilon^2)$ edges in $\tilde{O}(m\sqrt n/\epsilon^2)$ time. This improves upon the previous approximation factor $(8+\epsilon)$ of Chechik et al. for the same running time.

==> new_2approx_unw_pseudo.tex <==
\begin{breakablealgorithm}
{
\fontsize{9}{9}\selectfont
\caption{$2$-Approximation algorithm for the girth in unweighted graphs.}
\label{alg:highgirth}
\begin{algorithmic}[1]
%\SetKwProg{procedure}{Procedure}{}{}
\Procedure{HighGirth}{$G=(V,E)$}{
    Let $R\subseteq V$ be a uniform random sample of $100n^{3/4}\log n$ nodes.\; 
    \ForEach{$s\in R$}{
            Do BFS from $s$ in $G$\;
    }
    Let $g$ be the length of the shortest cycle found by the BFS searches.\;
    Return $g$.
    \EndProcedure
}

\label{alg:randsampunw}
%\SetKwProg{procedure}{Procedure}{}{}
\Procedure{RandomSamples}{$G=(v,E),i$}{
    \ForEach{$j\in \{1,\ldots,i\}$}{
        \ForEach{$k\in \{1,\ldots,2\log n\}$}{
            Let $S_{j,k}\subseteq V$ be a uniform random sample of $100\sqrt n \log n$ vertices.\;
            \ForEach{$s\in S_{j,k}$}{
                Do BFS to and from $s$ to compute for all $v$, $d(s,v)$ and $d(v,s)$.\;
            }
        }  
    }
    \ForEach{$u\in V$}{
        \ForEach{$j\in \{1,\ldots,i\}$}{
            $R^j(u)\leftarrow \emptyset$.\;
            \ForEach{$k\in \{1,\ldots,2\log n\}$}{
                $T_k^j(u)\leftarrow \{s\in S_{j,k}~|~d(u,s)\leq j \textrm{ and for all } y\in R^j(u):~d(s,y)\leq i\}$.\;
            
                \If{$|T_k^j(u)|< 10\log n$}{
                    $R^j(u)\leftarrow R^j(u)\cup T_k^j(u)$\;
                    Exit this loop (over $k$).
                 }
                \Else{
                    Let $R_k^j(u)$ be a uniform random sample of $10\log n$ nodes from $T_k^j(u)$.\;
                    $R^j(u)\leftarrow R^j(u)\cup R_k^j(u)$.\;
                }
            }
        }
    } Return the sets $R^j(u)$ for all $j\leq i$, $u\in V$, and $d(s,v),d(v,s)$ for all $s\in \cup_{j,k}S_{j,k}$ and $v\in V$.
  \EndProcedure 
}    
   
\label{alg:modbfs}
%\SetKwProg{procedure}{Procedure}{}{}
\Procedure{ModBFS}{$(G=(v,E),u,i,R^1(u),\ldots,R^i(u)), d(\cdot)$}{
    // $d(\cdot)$ contains $d(s,v),d(v,s)$ for all $s\in \cup_{j,k}S_{j,k}$ and $v\in V$.\;

    $Visited\leftarrow$ empty hash table\;
    $N_0\leftarrow \{u\}$\;
    $Visited.insert(u)$\;
    \ForEach{$j$ from $0$ to $i-1$}{
        $N_{j+1}\leftarrow$ empty linked list\;
        \ForEach{$x\in N_j$}{
            \If{for every $s\in R^j(u)$, $d(x,s)\leq i$}{
                \ForEach{$y$ s.t. $(x,y)\in E$ and $y\notin Visited$}{
                    \If{$y=u$}{
                        Stop and return $j+1$\;
                    }
                    $N_{j+1}.insert(y)$\;
                    $Visited.insert(y)$\;
                }
            }
        }
    }
    Return $\infty$ // No $\leq i$ length cycle found through $u$\;
\EndProcedure
}    

\label{alg:girthapp}
%\SetKwProg{procedure}{Procedure}{}{}
\Procedure{GirthApprox}{$(G=(V,E))$}{
    $g_{high}\leftarrow {HighGirth}(G)$\;
    
    Let $Q\subseteq V$ be a uniform random sample of $100n^{1/2}\log n$ nodes.\; 
    \ForEach{$s\in Q$}{
            Do BFS from and to $s$ in $G$\;
    }
    Let $i$ be the minimum integer s.t. $\exists s\in Q$ and $\exists v\in V$ with $d(s,v)\leq i+1$ and $d(v,s)\leq i+1$.\;
    $g_{med}\leftarrow 2(i+1)$\;
    
    Let $i$ be the min of $i$ and $n^{1/4}$\;
    
    Run ${RandomSamples}(G,i)$ to obtain sets $R^j(u)$ for all $j\leq i$, $u\in V$, and $d(\cdot)$ containing $d(s,v),d(v,s)$ for all $s\in \cup_{j,k}S_{j,k}$ and $v\in V$\;
    
    \ForEach{$u\in V$}{
        $g_u\leftarrow {ModBFS}(G,u,i,R^1(u),\ldots,R^i(u), d(\cdot))$\;
    }
    
    $g\leftarrow \min\{g_{high},g_{med}, \min_{u\in V} g_u\}$\;
    Return $g$\;
    \EndProcedure
}
\end{algorithmic}
}
\end{breakablealgorithm}

